Simons Lectures on Categorical Symmetries

Global Categorical Symmetries are a powerful new tool for analyzing quantum field theories. This volume compiles lecture notes from the 2022 and 2023 summer schools on Global Categorical Symmetries, held at the Perimeter Institute for Theoretical Physics and at the Swiss Map Research Station in Les Diableret. Specifically, this volume collects the lectures: * An introduction to symmetries in quantum field theory, Kantaro Ohmori * Introduction to anomalies in quantum field theory, Clay C\'ordova * Symmetry Categories 101, Michele Del Zotto * Applied Cobordism Hypothesis, David Jordan * Finite symmetry in QFT, Daniel S. Freed These volumes are devoted to interested newcomers: we only assume (basic) knowledge of quantum field theory (QFT) and some relevant maths. We try to give appropriate references for non-standard materials that are not covered. Our aim in this first volume is to illustrate some of the main questions and ideas together with some of the methods and the techniques necessary to begin exploring global categorical symmetries of QFTs.

==> Makefile <==
pdf := gcs-school-2022.pdf

ifdef batchmode
	latex-opts := -interaction batchmode
endif

SHELL := /bin/zsh
xopps := $(shell print xopp-figures-src/**/*.xopp(N))
xopp-pdfs := $(patsubst xopp-figures-src/%.xopp,xopp-figures/%.pdf,$(xopps))

deps := *.tex bibli.bib jheppub.sty JHEP.bst \
		clay-anomalies kantaro-sym dan \
		constantin michele-cat101 david \
		appendix \
		LesDiablerets.pdf LesDiablerets_white.pdf

.PHONY: clean clean-all
.ONESHELL:

$(pdf): sandbox/main.pdf
	cp sandbox/main.pdf $@

sandbox/main.pdf: $(deps) $(xopp-pdfs) sandbox
	cd sandbox
	[[ -e bibli.bcf ]] && bcf="$$(< bibli.bcf)"
	pdflatex $(latex-opts) main.tex
	if [[ -z "$$bcf" || "$$bcf" != "$$(< bibli.bcf)" ]]; then
		biber bibli.bcf
		pdflatex $(latex-opts) main.tex
	fi
	pdflatex $(latex-opts) main.tex

sandbox: *.tex
	mkdir -p sandbox
	ln -srf $(deps) xopp-figures sandbox

xopp-figures/%.pdf: xopp-figures-src/%.xopp
	mkdir -p "$(dir $@)"
	xournalpp --create-pdf="$@" "$<"

clean:
	rm -rf $(pdf) sandbox

clean-all: clean
	rm -rf xopp-figures


==> constantin/constantin.tex <==
% newcommands can go here

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcourse[Leon Liu and Luuk Stehouwer]{The Mathematics of TQFTs and Defects}{Constantin Teleman}


\section{section 1}

